Design and Evaluation of Deep Reinforcement Learning for Energy Saving in Open RAN

Next-generation wireless systems, already widely deployed, are expected to become even more prevalent in the future, representing challenges in both environmental and economic terms. This paper focuses on improving the energy efficiency of intelligent and programmable Open Radio Access Network (RAN) systems through the near-real-time dynamic activation and deactivation of Base Station (BS) Radio Frequency (RF) frontends using Deep Reinforcement Learning (DRL) algorithms, i.e., Proximal Policy Optimization (PPO) and Deep Q-Network (DQN). These algorithms run on the RAN Intelligent Controllers (RICs), part of the Open RAN architecture, and are designed to make optimal network-level decisions based on historical data without compromising stability and performance. We leverage a rich set of Key Performance Measurements (KPMs), serving as state for the DRL, to create a comprehensive representation of the RAN, alongside a set of actions that correspond to some control exercised on the RF frontend. We extend ns-O-RAN, an open-source, realistic simulator for 5G and Open RAN built on ns-3, to conduct an extensive data collection campaign. This enables us to train the agents offline with over 300,000 data points and subsequently evaluate the performance of the trained models. Results show that DRL agents improve energy efficiency by adapting to network conditions while minimally impacting the user experience. Additionally, we explore the trade-off between throughput and energy consumption offered by different DRL agent designs.

==> Reviewers_comments.tex <==
Camera-Ready Version Submission Deadline: 
November 15, 2024, 23:59:00 PDT 

REVIEWER 1
%1)  it is not clear how the DRL agent with input states from a dataset can take an action that shall generate a new state to feed it back to the agent for the next iteration, even with a very big dataset this should not be able to cover all the states with inner state parameters. % unclear question: this is how a DRL model works: apply an action that generates states and I use them to generate another action even if I never saw them 
%2) the reasons for selecting the state parameters are unclear in the paper, some parameters need more explanation related to RLF. Also, the author needs to elaborate and provide references for calculating the cost of BS activation. % more details on the RLF formula are already given and a reference on why we chose that states
3) the convergence and the complexity of the learning agents are missing in the evaluation section % He wants the WanDB plots

REVIEWER 2
1) The evaluation does not consider the energy consumed by the proposed system itself. % How much energy is the RL agent consuming?
When using DLR one question that arises is: what is the cost of the DLR both in computational terms and energy consumption? Or, putting it in another way: adding up the costs of DLR data collection (storage and networking), and training (and everything associated to it) with the energy spent in the system results in a lower energy consumption than a naive or heuristic approach? I.e., the energy consumption in Fig 3 should consider the energy consumed by the algorithms as well. 
% Idea for a journal extension?
2) The title does not mention the purpose of deep learning. Is it for managing specific aspects in Open-RAN? This could be clearer in the title (as in the abstract). % it is for energy saving in open ran
%3) The introduction does not make clear if/when real network setups allow the deactivation of RF frontends and in what proportion this happens in practice. It mentions "a dataset is generated through a large-scale campaign with thousands of simulations", but it is not clear if this dataset is completely synthetic or derived from real data. % In the introduction we are already saying that are simulations but we don't specify which software we are using, to fix
4) The state-of-the-art: What are the challenges this work does not cover that the proposal does? Why is DRL needed to solve these challenges? % we can add it 



REVIEWER 3
- Since offline DRL training has been used based on historical data, will this xApp be good to handle time varying RF environments in the near real time scale? % I don't understand: we are just applying actions to the RF 
%2) Typos: % to fix
    %- "...enabling dynamic infrastructure reconfigurations. This software-based approach allows the integration of xApps, which are algorithms designed to manage the RAN in real-time." >> xApps can manage the RAN in near-real time. 
    % - "The main contribution of this paper is the development of
    % a xApp" >> an xApp


GENERAL INFO    
When paper ready: 
Read this page again to check PDF quality and submission through EDAS
%https://ccnc2025.ieee-ccnc.org/authors/author-and-submission-guidelines 
A pdf-express generated file is mandatory to ensure that your paper will be uploaded on IEEE Xplore.

register for the conference at the full (non-student rate, member or non-member) rate BEFORE submitting the paper

PRESENTATION
20 min presentation with Questions
bring to the Session Chair a short bio

bring your portable computer with a VGA adaptor if required, or at least bring a copy of your presentation in a USB pen.

